FederatedTrust: A Solution for Trustworthy Federated Learning

The rapid expansion of the Internet of Things (IoT) and Edge Computing has presented challenges for centralized Machine and Deep Learning (ML/DL) methods due to the presence of distributed data silos that hold sensitive information. To address concerns regarding data privacy, collaborative and privacy-preserving ML/DL techniques like Federated Learning (FL) have emerged. However, ensuring data privacy and performance alone is insufficient since there is a growing need to establish trust in model predictions. Existing literature has proposed various approaches on trustworthy ML/DL (excluding data privacy), identifying robustness, fairness, explainability, and accountability as important pillars. Nevertheless, further research is required to identify trustworthiness pillars and evaluation metrics specifically relevant to FL models, as well as to develop solutions that can compute the trustworthiness level of FL models. This work examines the existing requirements for evaluating trustworthiness in FL and introduces a comprehensive taxonomy consisting of six pillars (privacy, robustness, fairness, explainability, accountability, and federation), along with over 30 metrics for computing the trustworthiness of FL models. Subsequently, an algorithm named FederatedTrust is designed based on the pillars and metrics identified in the taxonomy to compute the trustworthiness score of FL models. A prototype of FederatedTrust is implemented and integrated into the learning process of FederatedScope, a well-established FL framework. Finally, five experiments are conducted using different configurations of FederatedScope to demonstrate the utility of FederatedTrust in computing the trustworthiness of FL models. Three experiments employ the FEMNIST dataset, and two utilize the N-BaIoT dataset considering a real-world IoT security use case.

==> tablas_backup.tex <==

\begin{table}[t!]
\centering
\scriptsize
\begin{tabular}{|llll|} 
\hline
\rowcolor[rgb]{0.961,0.58,0.58} \textbf{trustworthiness score} & \textbf{0.56}         & \multicolumn{2}{l|}{}            \\ 
\hline
\rowcolor[rgb]{0.843,0.816,0.816} \textbf{robustness}          & \textbf{0.5}         & \multicolumn{2}{l|}{}            \\ 
\hline
resilience to attacks                                          & 0.48                  & certified robustness     & 0.48  \\ 
\hline
\multirow{2}{*}{algorithm robustness}                          & \multirow{2}{*}{0.035} & performance              & 0.07  \\
&                       & personalization          & 0     \\ 
\hline
client reliability                                             & 1                  & scale                    & 1  \\ 
\hline
\rowcolor[rgb]{0.816,0.804,0.804} \textbf{privacy}             & \textbf{0.31}         &                          &       \\ 
\hline
technique                                                      & 0                     & differential privacy     & 0     \\ 
\hline
uncertainty                                                    & 0.92                  & entropy                  & 0.92  \\ 
\hline
indistinguishability                                           & 0                     & global privacy risk      & 0     \\ 
\hline
\rowcolor[rgb]{0.827,0.812,0.812} \textbf{fairness}            & \textbf{0.25}         &                          &       \\ 
\hline
selection fairness                                             & 0.08                  & selection variation      & 0.08  \\ 
\hline
performance fairness                                           & 0.58                   & performance variation    & 0.58   \\ 
\hline
class distribution                                             & 0.08                  & class imbalance          & 0.08  \\ 
\hline
\rowcolor[rgb]{0.804,0.796,0.796} \textbf{explainability}      & \textbf{0.61}         &                          &       \\ 
\hline
\multirow{2}{*}{interpretability}                              & \multirow{2}{*}{0.55} & algorithmic transparency & 0.09  \\
&                       & model size               & 1     \\ 
\hline
post-hoc methods                                               & 0.67                  & feature importance       & 0.67  \\ 
\hline
\end{tabular}
\caption{Experiment 1 - 10 clients, 20\% sampling rate, 5 rounds, no DP}
\label{table:exp_1_result}
\end{table}






\begin{table}[t!]
\centering
\scriptsize
\begin{tabular}{|llll|} 
\hline
\rowcolor[rgb]{0.961,0.58,0.58} \textbf{trustworthiness score} & \textbf{0.65}         & \multicolumn{2}{l|}{}            \\ 
\hline
\rowcolor[rgb]{0.843,0.816,0.816} \textbf{robustness}          & \textbf{0.38}         & \multicolumn{2}{l|}{}            \\ 
\hline
resilience to attacks                                          & 0.19                  & certified robustness     & 0.19  \\ 
\hline
\multirow{2}{*}{algorithm robustness}                          & \multirow{2}{*}{0.05} & performance              & 0.1  \\
&                       & personalization          & 0     \\ 
\hline
client reliability                                             & 0.91                  & scale                    & 0.91  \\ 
\hline
\rowcolor[rgb]{0.816,0.804,0.804} \textbf{privacy}             & \textbf{0.64}         &                          &       \\ 
\hline
technique                                                      & 1                     & differential privacy     & 1     \\ 
\hline
uncertainty                                                    & 0.92                  & entropy                  & 0.92  \\ 
\hline
indistinguishability                                           & 0.0                  & global privacy risk      & 0.0  \\ 
\hline
\rowcolor[rgb]{0.827,0.812,0.812} \textbf{fairness}            & \textbf{0.47}         &                          &       \\ 
\hline
selection fairness                                             & 0.83                  & selection variation      & 0.83  \\ 
\hline
performance fairness                                           & 0.50                  & performance variation    & 0.50  \\ 
\hline
class distribution                                             & 0.08                  & class imbalance          & 0.08  \\ 
\hline
\rowcolor[rgb]{0.804,0.796,0.796} \textbf{explainability}      & \textbf{0.73}         &                          &       \\ 
\hline
\multirow{2}{*}{interpretability}                              & \multirow{2}{*}{0.55} & algorithmic transparency & 0.09  \\
&                       & model size               & 1     \\ 
\hline
post-hoc methods                                               & 0.92                  & feature importance       & 0.92  \\
\hline
\end{tabular}
\caption{Experiment 2 - 50 clients, 60\% sampling rate, 25 rounds, DP \(\epsilon\) = 20}
\label{table:exp_2_result}
\end{table}








\begin{table}[t!]
\centering
\scriptsize
\begin{tabular}{|llll|} 
\hline
\rowcolor[rgb]{0.961,0.58,0.58} \textbf{trustworthiness score} & \textbf{0.64}         & \multicolumn{2}{l|}{}            \\ 
\hline
\rowcolor[rgb]{0.843,0.816,0.816} \textbf{robustness}          & \textbf{0.36}         & \multicolumn{2}{l|}{}            \\ 
\hline
resilience to attacks                                          & 0.14                  & certified robustness     & 0.14  \\ 
\hline
\multirow{2}{*}{algorithm robustness}                          & \multirow{2}{*}{0.045} & performance              & 0.09  \\
&                       & personalization          & 0     \\ 
\hline
client reliability                                             & 0.91                  & scale                    & 0.91  \\ 
\hline
\rowcolor[rgb]{0.816,0.804,0.804} \textbf{privacy}             & \textbf{0.68}         &                          &       \\ 
\hline
technique                                                      & 1                     & differential privacy     & 1     \\ 
\hline
uncertainty                                                    & 0.92                  & entropy                  & 0.92  \\ 
\hline
indistinguishability                                           & 0.11                     & global privacy risk      & 0.11     \\ 
\hline
\rowcolor[rgb]{0.827,0.812,0.812} \textbf{fairness}            & \textbf{0.47}         &                          &       \\ 
\hline
selection fairness                                             & 0.83                  & selection variation      & 0.83  \\ 
\hline
performance fairness                                           & 0.50                   & performance variation    & 0.50   \\ 
\hline
class distribution                                             & 0.08                  & class imbalance          & 0.08  \\ 
\hline
\rowcolor[rgb]{0.804,0.796,0.796} \textbf{explainability}      & \textbf{0.65}         &                          &       \\ 
\hline
\multirow{2}{*}{interpretability}                              & \multirow{2}{*}{0.55} & algorithmic transparency & 0.09  \\
&                       & model size               & 1     \\ 
\hline
post-hoc methods                                               & 0.75                  & feature importance       & 0.75  \\ 
\hline
\end{tabular}
\caption{Experiment 3 - 50 clients, 60\% sampling rate, 20 rounds, DP \(\epsilon\) = 6}
\label{table:exp_3_result}
\end{table}







\begin{table}[t!]
\centering
\scriptsize
\begin{tabular}{|llll|} 
\hline
\rowcolor[rgb]{0.961,0.58,0.58} \textbf{trustworthiness score} & \textbf{0.67}         & \multicolumn{2}{l|}{}            \\ 
\hline
\rowcolor[rgb]{0.843,0.816,0.816} \textbf{robustness}          & \textbf{0.38}         & \multicolumn{2}{l|}{}            \\ 
\hline
resilience to attacks                                          & 0.05                  & certified robustness     & 0.05  \\ 
\hline
\multirow{2}{*}{algorithm robustness}                          & \multirow{2}{*}{0.18} & performance              & 0.36  \\
&                       & personalization          & 0     \\ 
\hline
client reliability                                             & 0.91                  & scale                    & 0.91  \\ 
\hline
\rowcolor[rgb]{0.816,0.804,0.804} \textbf{privacy}             & \textbf{0.71}         &                          &       \\ 
\hline
technique                                                      & 1                     & differential privacy     & 1     \\ 
\hline
uncertainty                                                    & 0.92                  & entropy                  & 0.92  \\ 
\hline
indistinguishability                                           & 0.20                  & global privacy risk      & 0.20  \\ 
\hline
\rowcolor[rgb]{0.827,0.812,0.812} \textbf{fairness}            & \textbf{0.50}         &                          &       \\ 
\hline
selection fairness                                             & 0.83                  & selection variation      & 0.83  \\ 
\hline
performance fairness                                           & 0.58                  & performance variation    & 0.58  \\ 
\hline
class distribution                                             & 0.08                  & class imbalance          & 0.08  \\ 
\hline
\rowcolor[rgb]{0.804,0.796,0.796} \textbf{explainability}      & \textbf{0.73}         &                          &       \\ 
\hline
\multirow{2}{*}{interpretability}                              & \multirow{2}{*}{0.55} & algorithmic transparency & 0.09  \\
&                       & model size               & 1     \\ 
\hline
post-hoc methods                                               & 0.92                  & feature importance       & 0.92  \\
\hline
\end{tabular}
\caption{Experiment 4 - 100 clients, 60\% sampling rate, 50 rounds, DP \(\epsilon\) = 6}
\label{table:exp_4_results}
\end{table}
